Large-scale Optimization with Linear Equality Constraints using Reduced Compact Representation

For optimization problems with linear equality constraints, we prove that the (1,1) block of the inverse KKT matrix remains unchanged when projected onto the nullspace of the constraint matrix. We develop reduced compact representations of the limited-memory inverse BFGS Hessian to compute search directions efficiently when the constraint Jacobian is sparse. Orthogonal projections are implemented by a sparse QR factorization or a preconditioned LSQR iteration. In numerical experiments two proposed trust-region algorithms improve in computation times, often significantly, compared to previous implementations of related algorithms and compared to IPOPT.

==> shared.tex <==
%------------------------------------ shared.tex ------------------------------------%
%
% Shared macros, definitions
%
%------------------------------------------------------------------------------------%
% 04/19/18 J.B command definitions

%\newcommand{\nl}{\vspace{0.5cm}} % newline 

%\renewcommand{\b}[1]{\ensuremath{\mathbf{#1}}} % bold
\renewcommand{\b}[1]{\ensuremath{#1}} % bold
%\newcommand{\bh}[1]{\ensuremath{\hat{\mathbf{#1}}}}
\newcommand{\bh}[1]{\ensuremath{\hat{#1}}}
\newcommand{\bti}[1]{\ensuremath{\tilde{\mathbf{#1}}}}
%\newcommand{\bk}[1]{\ensuremath{\mathbf{#1}_k}}
\newcommand{\bk}[1]{\ensuremath{{#1}_k}}
%\newcommand{\bko}[1]{\ensuremath{\mathbf{#1}_{k+1}}}
\newcommand{\bko}[1]{\ensuremath{{#1}_{k+1}}}
\newcommand{\bkmo}[1]{\ensuremath{\mathbf{#1}_{k-1}}}
%\newcommand{\bhk}[1]{\ensuremath{\widehat{\mathbf{#1}}_k}}
\newcommand{\bhk}[1]{\ensuremath{\widehat{#1}_k}}
\newcommand{\bi}[1]{\ensuremath{\mathbf{#1}^{-1}}}
%\newcommand{\bik}[2][1]{\ensuremath{\mathbf{#2}^{-#1}_k}}
\newcommand{\bik}[2][1]{\ensuremath{{#2}^{-#1}_k}}
\newcommand{\bhik}[2][1]{\ensuremath{\hat{\mathbf{#2}}^{-#1}_k}}
\newcommand{\bupklwX}[2][1]{\ensuremath{\mathbf{#2}^{(k)}_{#1}}}
\newcommand{\bz}[1]{\ensuremath{\mathbf{#1}_0}}

%\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\bs}[1]{\ensuremath{#1}}
\newcommand{\bsk}[1]{\ensuremath{\boldsymbol{#1}_k}}
\newcommand{\bshk}[1]{\ensuremath{\hat{\boldsymbol{#1}}_k}}

\newcommand{\bbk}[1]{\ensuremath{\bar{\mathbf{#1}}_k}}
\newcommand{\bb}[1]{\ensuremath{\bar{\mathbf{#1}}}}
\newcommand{\bbik}[2][1]{\ensuremath{\bar{\mathbf{#2}}^{-#1}_k}}

\newcommand{\bpo}[1]{\ensuremath{\mathbf{#1}_{\parallel 1}}}
\newcommand{\bp}[1]{\ensuremath{\mathbf{#1}_{\parallel }}}
\newcommand{\bpt}[1]{\ensuremath{\mathbf{#1}_{\parallel 2}}}
\newcommand{\bt}[1]{\ensuremath{\mathbf{#1}_{2}}}
\newcommand{\bo}[1]{\ensuremath{\mathbf{#1}_{1}}}
\newcommand{\bper}[1]{\ensuremath{\mathbf{#1}_{\perp}}}

\newcommand{\bbp}[1]{\ensuremath{\bar{\mathbf{#1}}_{\parallel}}}

\newcommand{\btk}[1]{\ensuremath{\tilde{\mathbf{#1}}_k}}
\newcommand{\btko}[1]{\ensuremath{\tilde{\mathbf{#1}}_{k+1}}}

%\newcommand{\biidx}[2]{\ensuremath{{\mathbf{#2}}_{#1}}}
\newcommand{\biidx}[2]{\ensuremath{#2}_{#1}}
\newcommand{\biidxh}[2]{\widehat{\ensuremath{#2}}_{#1}}

\newcommand{\bicidx}[2]{\ensuremath{{\mathbf{#2}}_{\bar{#1}}}}

\newcommand{\bkiidx}[2]{\ensuremath{{\mathbf{#2}}^{(k)}_{#1}}}

\newcommand{\bkoiidx}[2]{\ensuremath{{\mathbf{#2}}^{(k+1)}_{#1}}}

\newcommand{\jaciidx}[3]{\ensuremath{{ \nabla_{#1} \mathbf{#2}_{#3}}}}
\newcommand{\hessiidx}[2]{\ensuremath{\nabla^2_{#1 #2} }}

\newcommand{\bkoex}[2]{\ensuremath{\mathbf{#1}^{#2}_{k+1}}} % 03/13/19
\newcommand{\bkex}[2]{\ensuremath{\mathbf{#1}^{#2}_{k}}}

\newcommand{\bskoex}[2]{\ensuremath{\boldsymbol{#1}^{#2}_{k+1}}} % 03/13/19
\newcommand{\bskex}[2]{\ensuremath{\boldsymbol{#1}^{#2}_{k}}}
%\renewcommand{\bl}{\ensuremath{\mathbf{\mathcal{L}}}} 
\newcommand{\wh}[1]{\ensuremath{\widehat{#1}}}

\newcommand{\scjb}[1]{{\rmfamily\scshape #1}}

\newcommand{\bjex}[1]{\ensuremath{{\mathbf{#1}}^{(j)}}} % 03/31/20
\newcommand{\bjoex}[1]{\ensuremath{{\mathbf{#1}}^{(j+1)}}} % 03/31/20
\newcommand{\bbjex}[1]{\ensuremath{{\bar{\mathbf{#1}}}^{(j)}}} % 03/31/20
\newcommand{\bjzex}[1]{\ensuremath{{\mathbf{#1}}^{(0)}}} % 03/31/20

\newcommand{\tp}{^{\top}}   % 09/03/20
\newcommand{\mtp}{^{-\top}} % 11/19/20

\newcommand{\bks}[1]{\ensuremath{{#1}_k}(\sigma)} % 10/07/20 


